Gap junction plasticity as a mechanism to regulate network-wide oscillations

Cortical oscillations are thought to be involved in many cognitive functions and processes. Several mechanisms have been proposed to regulate oscillations. One prominent but understudied mechanism is gap-junctional coupling. Gap junctions are ubiquitous in cortex between GABAergic interneurons. Moreover, recent experiments indicate their strength can be modified in an activity-dependent manner, similar to chemical synapses. We hypothesized that activity-dependent gap junction plasticity acts as a mechanism to regulate oscillations in the cortex. We developed a computational model of gap junction plasticity in a recurrent cortical network. We showed that gap junction plasticity can serve as a homeostatic mechanism for oscillations by maintaining a tight balance between two network states: asynchronous irregular activity and synchronized oscillations. This homeostatic mechanism allows for robust communication between neuronal assemblies through two different mechanisms: transient oscillations and frequency modulation. This implies a direct functional role for gap junction plasticity in information transmission in cortex.

==> figure3-network.tex <==
%\documentclass[9pt,lineno]{elife}
%% \geometry{top=0.5in,left=0.50in,bottom=0.5in,right=0.50in}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage[utf8]{inputenc}
%%\usepackage[latin9]{inputenc}
%\usepackage{wrapfig}
%\usepackage{textcomp}
%\usepackage{amsmath}
%%\usepackage{amssymb}
%\usepackage{graphicx}
%\usepackage{esint}
%\usepackage{subscript}
%\usepackage{rotating}
%\usepackage{float}
%\usepackage{graphicx,kantlipsum,setspace}
%\usepackage{tikz}
%
%\usepackage{tikzscale}
%%\usepackage{fontspec}
%%\usepackage{pgf}
%\usepackage{pgfplots}
%\usepackage{import}
%
%
%\usepackage{caption}
%\captionsetup[table]{font={stretch=1.2}}    
%\captionsetup[figure]{font={stretch=1.2}}    
%\makeatletter
%\def\ps@pprintTitle{%
% \let\@oddhead\@empty
% \let\@evenhead\@empty
% \def\@oddfoot{\centerline{\thepage}}%
% \let\@evenfoot\@oddfoot}
%
%
%\usepackage{marginnote}
%\usepackage{lineno}
%
%\@ifundefined{showcaptionsetup}{}{%
% \PassOptionsToPackage{caption=false}{subfig}}
%\usepackage{subfig}
%\makeatother
%
%\renewcommand{\rmdefault}{lmodern}
%
%\usepackage{pgfplots}
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% ARTICLE SETUP
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\title{Gap junction plasticity as a quantitative mechanism to regulate network-wide oscillations}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% ARTICLE START
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\newlength\figureheight
%\newlength\figurewidth
%
%\begin{document}

\usetikzlibrary{matrix,chains,positioning,decorations.pathreplacing,arrows,arrows.meta}
\usetikzlibrary{matrix,positioning,calc}
\usetikzlibrary{decorations.pathmorphing}

\xdefinecolor{c1}{HTML}{4ED99C}
\xdefinecolor{Ecol}{HTML}{FF6868}
\xdefinecolor{Icol}{HTML}{3366cc}

\xdefinecolor{GN}{HTML}{66ccff}
\xdefinecolor{SN}{HTML}{9999cc}
\xdefinecolor{GAP}{HTML}{4ED99C}

\tikzstyle{Ecircle} = [draw, circle, minimum size=.7cm, fill=Ecol]
\tikzstyle{SNcircle} = [draw, circle, minimum size=.7cm, fill=SN]
\tikzstyle{GNcircle} = [draw, circle, minimum size=.7cm, fill=GN]

\begin{tikzpicture}
\node[Ecircle] (E1) at (0,-1) {E};
\node[GNcircle] (I1) at (0.7,-1.7) {I};
\node[GNcircle] (I2) at (1.3,-2.3) {I};
\node[GNcircle] (I3) at (1.9,-2.9) {I};
\node[GNcircle] (I4) at (2.5,-3.5) {I};

\node [
        draw, rectangle,
        anchor=north west,
        minimum width=3.5cm, minimum height=3.5cm,
        label=Gamma Network
      ] at (-0.5,-0.5) {};

\node [
        draw, rectangle,
        anchor=north west,
        color=GN,
        minimum width=2.7cm, minimum height=2.7cm,
      ] (GN) at (0.3,-1.3) {};

%\draw [GN] (0.3,-1.3) rectangle (3,-4);

\begin{scope} [color=GAP]
\path
(I1) edge [bend right=60] node {} (I2)
	edge [bend left=60] node {} (I3)
	edge [bend right=60] node {} (I4)
(I2) edge [bend left=60] node {} (I3)
	edge [bend right=60] node {} (I4)
(I3) edge [bend right=60] node {} (I4);
\end{scope}

\node [
        draw, rectangle,
        anchor=north west,
        minimum width=3.5cm, minimum height=3.5cm,
        label=Slow Network
      ] at (3,-4) {};
      

\node [
        draw, rectangle,
        anchor=north west,
        color=SN,
        minimum width=2.7cm, minimum height=2.7cm,
      ] (SN) at (3,-4) {};


\node[Ecircle] (E2) at (6,-7) {E};
\node[SNcircle] (I5) at (3.5,-4.5) {I};
\node[SNcircle] (I6) at (4.1,-5.1) {I};
\node[SNcircle] (I7) at (4.7,-5.7) {I};
\node[SNcircle] (I8) at (5.3,-6.3) {I};

\begin{scope} [color=GAP]
\path
(I5) edge [bend left=60] node {} (I6)
	edge [bend left=60] node {} (I7)
	edge [bend left=60] node {} (I8)
(I6) edge [bend right=60] node {} (I7)
	edge [bend right=60] node {} (I8)
(I7) edge [bend left=60] node {} (I8);
\end{scope}

\begin{scope}   [dashed,color=GAP] 
\path
	(I3) edge [bend left=60] node {} (I5)
	(I6) edge [bend left=60] node {} (I4)
	(I4) edge node {} (I5);
\end{scope}

\path
	(E1) edge [bend left=50,-triangle 90 reversed] node {} (GN)
	(E1) edge [bend right=50,*-] node {} (GN)
	(E2) edge [bend left=50,-triangle 90 reversed] node {} (SN)
	(E2) edge [bend right=50,*-] node {} (SN);
	
    
\end{tikzpicture}
%\textsl{•}\end{document}
